Fuzzy c-Means Clustering for Persistence Diagrams

Persistence diagrams concisely represent the topology of a point cloud whilst having strong theoretical guarantees, but the question of how to best integrate this information into machine learning workflows remains open. In this paper we extend the ubiquitous Fuzzy c-Means (FCM) clustering algorithm to the space of persistence diagrams, enabling unsupervised learning that automatically captures the topological structure of data without the topological prior knowledge or additional processing of persistence diagrams that many other techniques require. We give theoretical convergence guarantees that correspond to the Euclidean case, and empirically demonstrate the capability of our algorithm to capture topological information via the fuzzy RAND index. We end with experiments on two datasets that utilise both the topological and fuzzy nature of our algorithm: pre-trained model selection in machine learning and lattices structures from materials science. As pre-trained models can perform well on multiple tasks, selecting the best model is a naturally fuzzy problem; we show that fuzzy clustering persistence diagrams allows for model selection using the topology of decision boundaries. In materials science, we classify transformed lattice structure datasets for the first time, whilst the probabilistic membership values let us rank candidate lattices in a scenario where further investigation requires expensive laboratory time and expertise.

==> ICML 2021/tikz_fig.tex <==
\begin{tikzpicture}[scale=2]
\draw[fill](0.9600173033359185, 0.699512049949576) circle[radius = 1pt];
\draw[fill](0.9998672926238792, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](0.361056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](0.996455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](0.13654457982352464, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](0.3205192835651931, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](0.7096515625881274, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](0.5341154391977205, 0.24729376490994515) circle[radius = 1pt];
\draw [thick] (2.499867292623879,0.22006729978285178)--(2.496455725089097,0.3163469777906084);
\draw [thick] (1.6365445798235245,0.3839800101516001)--(1.820519283565193,0.3664147530835151);
\draw [thick] (1.820519283565193,0.3664147530835151)--(2.0341154391977208,0.24729376490994515);
\draw [thick] (2.4600173033359187,0.699512049949576)--(2.2096515625881272,0.9001424305233735);
\draw [thick] (1.861056353964058,0.739840990209437)--(1.820519283565193,0.3664147530835151);
\draw [thick] (1.861056353964058,0.739840990209437)--(2.2096515625881272,0.9001424305233735);
\draw [thick] (2.4600173033359187,0.699512049949576)--(2.496455725089097,0.3163469777906084);
\draw[fill](2.4600173033359187, 0.699512049949576) circle[radius = 1pt];
\draw[fill](2.499867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](1.861056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](2.496455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](1.6365445798235245, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](1.820519283565193, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](2.2096515625881272, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](2.0341154391977208, 0.24729376490994515) circle[radius = 1pt];
\draw [thick, fill=blue!65] (3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151);
\draw [thick, fill=blue!65] (3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.9600173033359187,0.699512049949576)--(3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084);
\draw [thick] (3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151);
\draw [thick] (3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.7096515625881272,0.9001424305233735);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.320519283565193,0.3664147530835151);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.7096515625881272,0.9001424305233735);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.996455725089097,0.3163469777906084);
\draw [thick] (3.1365445798235245,0.3839800101516001)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001);
\draw [thick] (3.999867292623879,0.22006729978285178)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.996455725089097,0.3163469777906084)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.999867292623879,0.22006729978285178);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.5341154391977208,0.24729376490994515);
\draw[fill](3.9600173033359187, 0.699512049949576) circle[radius = 1pt];
\draw[fill](3.999867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](3.361056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](3.996455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](3.1365445798235245, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](3.320519283565193, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](3.7096515625881272, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](3.5341154391977208, 0.24729376490994515) circle[radius = 1pt];
\draw [thick, fill=blue!65] (4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151);
\draw [thick, fill=blue!65] (5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437)--(5.209651562588127,0.9001424305233735);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084)--(5.209651562588127,0.9001424305233735);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151)--(5.209651562588127,0.9001424305233735);
\draw [thick] (5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084);
\draw [thick] (4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151);
\draw [thick] (4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.209651562588127,0.9001424305233735);
\draw [thick] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151);
\draw [thick] (4.861056353964058,0.739840990209437)--(5.209651562588127,0.9001424305233735);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084);
\draw [thick] (4.636544579823525,0.3839800101516001)--(5.034115439197721,0.24729376490994515);
\draw [thick] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001);
\draw [thick] (5.499867292623879,0.22006729978285178)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178);
\draw [thick] (4.861056353964058,0.739840990209437)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.496455725089097,0.3163469777906084)--(5.209651562588127,0.9001424305233735);
\draw [thick] (4.8205192835651935,0.3664147530835151)--(5.209651562588127,0.9001424305233735);
\draw[fill](5.460017303335919, 0.699512049949576) circle[radius = 1pt];
\draw[fill](5.499867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](4.861056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](5.496455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](4.636544579823525, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](4.8205192835651935, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](5.209651562588127, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](5.034115439197721, 0.24729376490994515) circle[radius = 1pt];
\end{tikzpicture}
 \linebreak 


==> tikz_fig.tex <==
\begin{tikzpicture}[scale=2]
\draw[fill](0.9600173033359185, 0.699512049949576) circle[radius = 1pt];
\draw[fill](0.9998672926238792, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](0.361056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](0.996455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](0.13654457982352464, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](0.3205192835651931, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](0.7096515625881274, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](0.5341154391977205, 0.24729376490994515) circle[radius = 1pt];
\draw [thick] (2.499867292623879,0.22006729978285178)--(2.496455725089097,0.3163469777906084);
\draw [thick] (1.6365445798235245,0.3839800101516001)--(1.820519283565193,0.3664147530835151);
\draw [thick] (1.820519283565193,0.3664147530835151)--(2.0341154391977208,0.24729376490994515);
\draw [thick] (2.4600173033359187,0.699512049949576)--(2.2096515625881272,0.9001424305233735);
\draw [thick] (1.861056353964058,0.739840990209437)--(1.820519283565193,0.3664147530835151);
\draw [thick] (1.861056353964058,0.739840990209437)--(2.2096515625881272,0.9001424305233735);
\draw [thick] (2.4600173033359187,0.699512049949576)--(2.496455725089097,0.3163469777906084);
\draw[fill](2.4600173033359187, 0.699512049949576) circle[radius = 1pt];
\draw[fill](2.499867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](1.861056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](2.496455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](1.6365445798235245, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](1.820519283565193, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](2.2096515625881272, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](2.0341154391977208, 0.24729376490994515) circle[radius = 1pt];
\draw [thick, fill=blue!65] (3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151);
\draw [thick, fill=blue!65] (3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.9600173033359187,0.699512049949576)--(3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001)--(3.5341154391977208,0.24729376490994515);
\draw [thick, fill=blue!65] (3.361056353964058,0.739840990209437)--(3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.999867292623879,0.22006729978285178)--(3.996455725089097,0.3163469777906084);
\draw [thick] (3.1365445798235245,0.3839800101516001)--(3.320519283565193,0.3664147530835151);
\draw [thick] (3.320519283565193,0.3664147530835151)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.7096515625881272,0.9001424305233735);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.320519283565193,0.3664147530835151);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.7096515625881272,0.9001424305233735);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.996455725089097,0.3163469777906084);
\draw [thick] (3.1365445798235245,0.3839800101516001)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.1365445798235245,0.3839800101516001);
\draw [thick] (3.999867292623879,0.22006729978285178)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.996455725089097,0.3163469777906084)--(3.5341154391977208,0.24729376490994515);
\draw [thick] (3.9600173033359187,0.699512049949576)--(3.999867292623879,0.22006729978285178);
\draw [thick] (3.361056353964058,0.739840990209437)--(3.5341154391977208,0.24729376490994515);
\draw[fill](3.9600173033359187, 0.699512049949576) circle[radius = 1pt];
\draw[fill](3.999867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](3.361056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](3.996455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](3.1365445798235245, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](3.320519283565193, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](3.7096515625881272, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](3.5341154391977208, 0.24729376490994515) circle[radius = 1pt];
\draw [thick, fill=blue!65] (4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151);
\draw [thick, fill=blue!65] (5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437)--(5.209651562588127,0.9001424305233735);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick, fill=blue!65] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084)--(5.209651562588127,0.9001424305233735);
\draw [thick, fill=blue!65] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151)--(5.209651562588127,0.9001424305233735);
\draw [thick] (5.499867292623879,0.22006729978285178)--(5.496455725089097,0.3163469777906084);
\draw [thick] (4.636544579823525,0.3839800101516001)--(4.8205192835651935,0.3664147530835151);
\draw [thick] (4.8205192835651935,0.3664147530835151)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.209651562588127,0.9001424305233735);
\draw [thick] (4.861056353964058,0.739840990209437)--(4.8205192835651935,0.3664147530835151);
\draw [thick] (4.861056353964058,0.739840990209437)--(5.209651562588127,0.9001424305233735);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.496455725089097,0.3163469777906084);
\draw [thick] (4.636544579823525,0.3839800101516001)--(5.034115439197721,0.24729376490994515);
\draw [thick] (4.861056353964058,0.739840990209437)--(4.636544579823525,0.3839800101516001);
\draw [thick] (5.499867292623879,0.22006729978285178)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.496455725089097,0.3163469777906084)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.499867292623879,0.22006729978285178);
\draw [thick] (4.861056353964058,0.739840990209437)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.460017303335919,0.699512049949576)--(4.861056353964058,0.739840990209437);
\draw [thick] (5.460017303335919,0.699512049949576)--(5.034115439197721,0.24729376490994515);
\draw [thick] (5.496455725089097,0.3163469777906084)--(5.209651562588127,0.9001424305233735);
\draw [thick] (4.8205192835651935,0.3664147530835151)--(5.209651562588127,0.9001424305233735);
\draw[fill](5.460017303335919, 0.699512049949576) circle[radius = 1pt];
\draw[fill](5.499867292623879, 0.22006729978285178) circle[radius = 1pt];
\draw[fill](4.861056353964058, 0.739840990209437) circle[radius = 1pt];
\draw[fill](5.496455725089097, 0.3163469777906084) circle[radius = 1pt];
\draw[fill](4.636544579823525, 0.3839800101516001) circle[radius = 1pt];
\draw[fill](4.8205192835651935, 0.3664147530835151) circle[radius = 1pt];
\draw[fill](5.209651562588127, 0.9001424305233735) circle[radius = 1pt];
\draw[fill](5.034115439197721, 0.24729376490994515) circle[radius = 1pt];
\end{tikzpicture}
 \linebreak 

